HeAL3D: Heuristical-enhanced Active Learning for 3D Object Detection

Active Learning has proved to be a relevant approach to perform sample selection for training models for Autonomous Driving. Particularly, previous works on active learning for 3D object detection have shown that selection of samples in uncontrolled scenarios is challenging. Furthermore, current approaches focus exclusively on the theoretical aspects of the sample selection problem but neglect the practical insights that can be obtained from the extensive literature and application of 3D detection models. In this paper, we introduce HeAL (Heuristical-enhanced Active Learning for 3D Object Detection) which integrates those heuristical features together with Localization and Classification to deliver the most contributing samples to the model's training. In contrast to previous works, our approach integrates heuristical features such as object distance and point-quantity to estimate the uncertainty, which enhance the usefulness of selected samples to train detection models. Our quantitative evaluation on KITTI shows that HeAL presents competitive mAP with respect to the State-of-the-Art, and achieves the same mAP as the full-supervised baseline with only 24% of the samples.

==> 05_discussion.tex <==
\section{Discussion}
\label{sec:discussion}
\todo{Sury and Esteban after results are there}

\todo{Future work: Semi supervised/Pseudo labels}

==> comments.tex <==
Major Weaknesses:

The proposed method is technically sound. However, it does not introduce new concepts or insights. Incorporating the number of points per box hampers active learning performance instead of improving it. For me, it is unclear why the paper contains this "contribution" when it does not positively contribute to the method.

The major weakness, however, is the weak evaluation:

    The KITTI dataset contains only three different object classes and a minimal number of frames covering only a small spatial area
    It is only labeled in the front view
    The ablation study does not show a range evaluation, or evaluation w.r.t. number of points per object which would support the claimed contributions
    The selection of the augmentation is not ablated.

To 1), 2), and 4): If there are labels available for the whole view (360 degrees), it is expected that a rotation of about 180 degrees would not reveal a very high uncertainty, especially for voxel-based detectors since the quantization of the point cloud would not change. Therefore, an evaluation with one of the state-of-the-art datasets, Waymo Open Dataset, NuScenes, ONCE, or Argoverse 2, is required to make better assumptions.
Minor Weaknesses:

In the following, I list some minor weaknesses which should be considered:

    [L186] The paper claims not to use additional forward passes. However, the proposed method also needs an additional forward pass (with the augmented version)
    [L229-L231] "for 3D object detection, localization is the greatest challenge": This statement requires proof from another paper or an empirical experiment!
    [L250-L253] The selection of this augmentation is not validated. This would require an ablation. Mirroring and rotation about another angle would also be a real scenario. Further, the 180° rotation is problematic for KITTI since labels are only available for the front view. This does not guarantee that the method would also work on other datasets or for 360° datasets.

Overall Recommendation: 1: reject
Justification For Recommendation And Suggestions For Rebuttal:

The topic of active learning in 3D LiDAR point clouds is important since labeling is expensive, and all methods mitigating this issue are valuable. However, the proposed method offers no new scientific methods or insights. The extremely poor evaluation on a relatively small and unbalanced dataset reveals that frames with underrepresented classes should be annotated. In addition, comparing a rotated scene by 180 degrees was chosen to calculate the uncertainty. This may work for a dataset like KITTI, where only the FOV is annotated, but it does not guarantee that it will work for 360-degree datasets, e.g., Waymo or NuScenes. An ablation study of the choice of augmentation techniques is also missing. The lack of novel methods and a limited evaluation with no new insights led to my decision to reject the paper.
Confidence Level: 4: High Confidence - The reviewer has strong expertise in the area. They are highly familiar with the relevant literature and can critically evaluate the paper.
Additional Comments For Authors:

In the following, I would like to point out unclear points that may help to improve the paper in the future:

    Question on how to calculate the probability map for classification? Does the class PDF also depend on the box's l,w, and h?
    [L455] Why is the training on batch size 1? The GPU memory can't be the limitation here.
    The teaser figure is of low quality. The motivation also indicates that a low number of points is a good indicator of important objects. However, this has not been shown in the results.
    Section 3.7 does not add value to the paper. It is unclear if the method requires multiple (at least 2) forward passes.

Major Weaknesses:

Generalization of the Approach:

    The evaluation misses an evaluation of the generalization of the approach. The Kitti dataset is a small dataset, e.g., reference [22] uses also the Waymo dataset and additionally 2D object detection. The strength of the approach lies in its applicability to any pretrained detection network and any dataset. Further studies on larger datasets, on a set of different object detection networks, or different detection tasks would show its potential to generalize beyond active learning for small datasets.

Heuristic Uncertainty or Informativeness Criterion:

    Within recent years, a large amount of works in computer vision and machine learning have addressed uncertainty quantification for deep neural networks. Early works used the difference in detections for the original view and augmented views as an approximation for uncertainty. The majority of today’s works use Bayesian approaches, ensembles, deterministic uncertainty methods, … etc. Considering this large amount of uncertainty estimation techniques, a passage on how the proposed uncertainty is embedded into the related works is missing. Are there similarities to deterministic uncertainty methods? What are related uncertainty metrics for object detection based on heuristics?
    An evaluation of the quality of the proposed uncertainty is missing. For this, the ECE metric is commonly computed. The proposed uncertainty metric is only evaluated within the context of active learning. This leaves the question open whether the heuristic measure is useful as a general uncertainty metric that can be used also for other tasks, or whether it performs well only as an informativeness measure in the context of active learning.

Minor Weaknesses:

Missing Clarity

    A section on the limitation of the approach is missing.
    L68,69: “It is therefore evident that objects for which the model is less confident should provide the most value …” References for this statement in the context of active learning are missing.

Evaluation

    Sec. 3.1 defines in line 244-246 the problem definition for an active learning pipeline as having a small, labeled dataset D_L with m samples and a large pool of unlabeled data D_U with n samples, where m << n. For Kitti, this work uses 900 samples for the active learning pipeline out of a total of 3.716 training samples. How many samples m are used to begin the active learning pipeline with a small labeled dataset?


Major Weaknesses:

    In section 3.6.2, line 442 states “we employ Average Precision (AP) for both 3D object detection, and the evaluation difficulty is categorized...”. It seems that the second task that uses AP as its evaluation metric has been omitted, since the word “both” is used, or it might just be a typo?

    In the referenced state-of-the-art KECOR and CRB papers, more than 1000 samples have been queried from the KITTI dataset, while the author has only queried up to 900. For a fair comparison, more samples could be queried, and more datasets could be used, such as the Waymo Open dataset.

    Would be good to add the pseudocode of the algorithm to the paper/supp.

    Can you please clarify the loss functions used in training the 3D object detector?

Minor Weaknesses:

    The figure of typical driving scenario for an autonomous vehicle and the caption in the introduction section is not very clear.

    Section 3.7 repeats and rephrases the same fact about the PV-RCNN model in the 2nd and 3rd sentences.

    Some spelling and grammatical errors in lines 377 (wrong instead of wrongly or incorrectly), 442 (“both” seems to be a typo), 509 (for them it is easier), 545 (vainilla instead of vanilla).

Overall Recommendation: 3: borderline
Justification For Recommendation And Suggestions For Rebuttal:

The paper used Gaussian Mixture Models to represent the object detection predictions, and KL divergence for uncertainty estimation between original and augmented predictions, which have both been done separately in previous papers. I added some weaknesses in describing how heuristic features are added to the final uncertainty estimation and selection threshold, and the lack of an algorithm pseudocode mentioned. Please see my comments above.

Also, I had a couple of questions.

    The methodology seems sound, but more information may be needed on how the distance and point uncertainty in Equation 8 (line 418) are incorporated to achieve the final uncertainty estimation metric, and its selection criteria and thresholds to decide whether the divergence is significant.

    Is the number of labeled samples on the x axis of the result figures the same as the number of selected bounding boxes used in the previous state-of-the-art approaches?



==> latexmkrc <==
add_cus_dep( 'tex', 'aux', 0, 'makeexternaldocument' );

sub makeexternaldocument {
    # if the dependency isn't one of the files that this latexmk run will consider, process it
    # without this test, we would get an infinite loop!
    if (!($root_filename eq $_[0]))
    {   # PLEASE ENABLE ONLY ONE OF THE FOLLOWING
        # DEPENDING ON THE ENGINE YOU'RE USING
    
        # FOR PDFLATEX
        system( "latexmk -pdf \"$_[0]\"" );

        # FOR LATEX+DVIPDF
        # system( "latexmk \"$_[0]\"" );

        # FOR XELATEX
        # system( "latexmk -xelatex \"$_[0]\"" );
        
        # FOR LUALATEX
        # system( "latexmk -lualatex \"$_[0]\"" );
   }
}

